A Confidence-based Iterative Solver of Depths and Surface Normals for Deep Multi-view Stereo

In this paper, we introduce a deep multi-view stereo (MVS) system that jointly predicts depths, surface normals and per-view confidence maps. The key to our approach is a novel solver that iteratively solves for per-view depth map and normal map by optimizing an energy potential based on the locally planar assumption. Specifically, the algorithm updates depth map by propagating from neighboring pixels with slanted planes, and updates normal map with local probabilistic plane fitting. Both two steps are monitored by a customized confidence map. This solver is not only effective as a post-processing tool for plane-based depth refinement and completion, but also differentiable such that it can be efficiently integrated into deep learning pipelines. Our multi-view stereo system employs multiple optimization steps of the solver over the initial prediction of depths and surface normals. The whole system can be trained end-to-end, decoupling the challenging problem of matching pixels within poorly textured regions from the cost-volume based neural network. Experimental results on ScanNet and RGB-D Scenes V2 demonstrate state-of-the-art performance of the proposed deep MVS system on multi-view depth estimation, with our proposed solver consistently improving the depth quality over both conventional and deep learning based MVS pipelines. Code is available at https://github.com/thuzhaowang/idn-solver.

==> latex/abstract_v0.tex <==
We present a method that iteratively solves for per-view depth map and normal map by optimizing an energy potential based upon the local planar assumption. Specifically, the algorithm updates depth map by propagating from neighboring pixels with slanted planes, and updates normal map with local probabilistic plane fitting. Both two steps are monitored by a customized confidence map. The proposed method is not only effective as a postprocessing tool for plane-based depth refinement and completion, but also differentiable such that it can be integrated into deep learning pipelines. We further introduce a deep multi-view stereo (MVS) system that predicts depth, normal and confidence jointly followed by the proposed confidence-based iterative depth-normal solver module. The whole system can be trained end-to-end, decoupling the challenging problem of matching pixels within textureless regions from the initial depth and normal predictions. Experiments show that the proposed solver consistently improves the depth quality over both conventional and deep learning based MVS pipelines. Results on ScanNet and RGBD Scenes demonstrate state-of-the-art performance of our proposed deep MVS system on multi-view depth estimation.


==> latex/related.tex <==

\paragraph{Multi-view Stereo.}
Reconstructing 3D models from posed images has been widely studied over decades. Early methods \cite{kutulakos2000theory, faugeras2002variational,vogiatzis2005multi} utilize volumetric optimization. Later attempts \cite{yoon2006adaptive,gallup2007real,bleyer2011patchmatch,hosni2012fast,schonberger2016pixelwise} reconstruct per-view depth maps by comparing cross-view image patches, which becomes the de facto approach of modern multi-view stereo pipelines. Recent advances include employing superpixels \cite{romanoni2019tapa}, post-refinement \cite{kuhn2019plane,kuhn2020deepc}, and advanced propagation checkerboards \cite{galliani2015massively,xu2019multi,xu2020planar}, etc. With the success of deep learning, a number of learning-based techniques are proposed to tackle the problem. While several methods learn to directly predict 3D geometry as grids \cite{kar2017learning,ji2017surfacenet}, point clouds \cite{chen2019point} and TSDF \cite{murez2020atlas}, per-view depth map estimation is still the top choice of most approaches \cite{wang2018mvdepthnet,yao2018mvsnet,im2019dpsnet,liu2019neural,hou2019multi,kusupati2020normal,long2020occlusion,duzcceker2020deepvideomvs,patil2020don} due to its robustness and flexibility. Most of those methods follow the spirit of conventional approaches \cite{gallup2007real,bleyer2011patchmatch} and train a cost volume based neural network. Some of the methods \cite{hou2019multi,duzcceker2020deepvideomvs,patil2020don} also integrate temporal information with recurrent networks. However, direct prediction over poorly textured areas have been one of the main difficulties of most approaches relying on cost volumes. An exception of this is DELTAS \cite{sinha2020deltas}, which proposes to learn interest points and perform triangulation and densification over sparse points. In this work, we also focus on per-view depth estimation and introduce an end-to-end MVS system equipped with a novel iterative solver. Our system implicitly decouples depth prediction over texture-less areas from the cost-volume based network, surpassing both leading cost-volume based methods and DELTAS \cite{sinha2020deltas} on multiple benchmarks. 

\vspace{-10pt}
\paragraph{Confidence Estimation.}
Accurately estimating per-view depth map confidence is beneficial to 3D reconstruction pipelines.
% , especially when dynamic programming methods are used for stereo optimization \cite{van2002hierarchical}. Conventionally confidence can be directly acquired from the computed similarity of cross-view local patches at different depths. 
Early confidence measures such as matching cost, peak ratio and maximum likelihood are extensively studied in \cite{hirschmuller2008evaluation,hu2012quantitative}. Local smoothness can also contribute to the confidence measurement of the stereo problem in  \cite{sun2003stereo, hirschmuller2007stereo}. Recently, learning-based methods \cite{seki2016patch,poggi2016learning} are proved to be effective on confidence estimation. Most related to us, \cite{kuhn2020deepc} exploits the counter map acquired from the geometric consistency check for deep confidence prediction. In our MVS system, we combine the deep confidence estimation and the geometric consistency based confidence estimation together to get our final confidence map, which monitors our iterative depth-normal solver at inference. 

\vspace{-10pt}
\paragraph{Depth-Normal Constraints.}
As depths and surface normals are naturally coupled by local plane fitting, joint depth-normal constraints are widely employed. Markov random fields with slanted-plane models were initially introduced in \cite{birchfield1999multiway}, and were later used in many stereo techniques \cite{hong2004segment,bleyer2005layered,yamaguchi2012continuous}. Those methods operate on superpixels and prefer locally planar surfaces. \cite{bleyer2011patchmatch} proposed to employ slanted support windows in its PatchMatch stereo framework, coupling the depth propagation with the randomly initialized per-pixel surface normal. \cite{valentin2018depth} propose to embed bilateral filtering in the plane fitting process to encourage locally planar structures of the output depth map. Recent learning-based methods also exploit surface normals to help train the depth prediction. While \cite{eigen2015predicting,qi2018geonet,kusupati2020normal} jointly predict depths and surface normals together to benefit from multi-task feature learning, recent literature \cite{yin2019enforcing,long2020occlusion} adopts online fitting, aiming to enrich the network with planar priors by supervising the fitted surface normals. In \cite{zhang2018deep}, a surface normal network is trained to help solve for dense depth map from sparse depth observations. Different from prior works, we present a new method to exploit depth-normal constraints via a differentiable iterative solver, which explicitly models local planar assumption in our deep MVS system. 


